Adaptive Prompting for Continual Relation Extraction: A Within-Task Variance Perspective

To address catastrophic forgetting in Continual Relation Extraction (CRE), many current approaches rely on memory buffers to rehearse previously learned knowledge while acquiring new tasks. Recently, prompt-based methods have emerged as potent alternatives to rehearsal-based strategies, demonstrating strong empirical performance. However, upon analyzing existing prompt-based approaches for CRE, we identified several critical limitations, such as inaccurate prompt selection, inadequate mechanisms for mitigating forgetting in shared parameters, and suboptimal handling of cross-task and within-task variances. To overcome these challenges, we draw inspiration from the relationship between prefix-tuning and mixture of experts, proposing a novel approach that employs a prompt pool for each task, capturing variations within each task while enhancing cross-task variances. Furthermore, we incorporate a generative model to consolidate prior knowledge within shared parameters, eliminating the need for explicit data storage. Extensive experiments validate the efficacy of our approach, demonstrating superior performance over state-of-the-art prompt-based and rehearsal-free methods in continual relation extraction.

==> Tables/abl-res.tex <==
\begin{table*} [t]
\small
\centering
    \begin{tabular}{l | c c c c c c c c c c} 
    \hline
    \multicolumn{11}{c}{\textbf{TACRED}} \\
    \hline
    Model & T1 & T2 & T3 & T4 & T5 & T6 & T7 & T8 & T9 & T10 \\
    \hline
    WAVE-CRE & \textbf{98.4} & \textbf{94.3} & \textbf{90.2} & \textbf{86.2} & 84.7 & \textbf{82.6} & \textbf{81.3} & \textbf{79.7} & \textbf{79.5} & \textbf{78.3} \\
    w/o Prompt Pool & 97.7 & 93.6 & 89.9 & 85.4 & 83.7 & 81.4 & 80.0 & 78.9 & 78.5 & 77.3 \\
    w/o Relation Classifier & \textbf{98.4}	& 94.1 & 89.4 &	85.7 &	\textbf{85.4} &	81.2 &	79.3 &	77.3 &	76.5 &	75.2 \\
    w/o Task ID & \textbf{98.4} & 52.6 & 37.8 & 27.3 & 22.6 & 18.6 & 15.1 & 14.5 & 12.7 & 11,5  \\
    w/o Task ID + Relation Classifier & \textbf{98.4} &	48.0 &	31.5 &	25.9 &	22.7 &	18.5 &	14.7 &	14.0 &	12.4 & 11.6 \\
    % \textbf{Ours} w/o SWAG & 98.3 & 94.2 & 90.0 & 86.0 & 84.5 & 82.1 & 80.5 & 78.6 & 78.4 & 77.3 \\
    \hline
    \end{tabular}
\caption{Ablation study of WAVE-CRE with three components: prompt pool for each task, generative models for training the task predictor, and generative models for the relation classifier.}
\label{tab:ablation_study}
\end{table*}



% \begin{table*} [ht]
% \small
% \centering
%     \begin{tabular}{c c c | c c c c c c c c c c} 
%     \hline
%     \multicolumn{13}{c}{Class Incremental Learning (TACRED)} \\
%     \hline
%     Top K & Prompt length & Pool size & T1 & T2 & T3 & T4 & T5 & T6 & T7 & T8 & T9 & T10 \\
%     \hline
%         1 & 8 & 10 & 97.2	&94.7	&91.2	&90.3	&88.6	&84.9	&77.7	&77.4	&76.0	&75.5 \\
%     4 & 2 & 40 & 97.2	&94.7	&91.2	&89.6	&88.0	&84.5	&78.2	&77.7	&76.2	&74.5 \\

%     8 & 1 & 80 & \textbf{98.2}	&\textbf{95.4}	&\textbf{92.0}	&\textbf{91.9}	&\textbf{89.6}	&\textbf{85.9}	&\textbf{81.2}	&\textbf{80.1}	&\textbf{78.4}	&\textbf{78.2} \\
%     \hline
%     \end{tabular}
%     \begin{tabular}{c c c | c c c c c c c c c c} 
%     \hline
%     \multicolumn{13}{c}{Task Incremental Learning (TACRED)} \\
%     \hline
%     Top K & Prompt length & Pool size & T1 & T2 & T3 & T4 & T5 & T6 & T7 & T8 & T9 & T10 \\
%     \hline
%     1 & 8 & 10 &\textbf{97.2}	&\textbf{95.5}	&93.1	&92.3	&90.5	&87.8	&84.6	&84.1	&83.4	&84.2 \\
%     4 & 2 & 40 & 96.5	&\textbf{95.5}	&92.1	&93.2	&91.2	&88.9	&85.3	&85.2	&76.2	&84.0 \\
%     8 & 1 & 80 & 96.5	&\textbf{95.5}	&\textbf{94.3}	&\textbf{94.1}	&\textbf{92.7}	&\textbf{90.0}	&\textbf{88.3}	&\textbf{87.7}	&\textbf{86.5}	&\textbf{85.2} \\
%     \hline
%     \end{tabular}
% \caption{Ablation study on the number of prompts used. We report the performance on TACRED, in two scenarios: Class-Incremental Learning and Task-Incremental Learning.}  
% \label{tab:abl-res}
% \end{table*}

==> checklist.tex <==
\section*{Reproducibility Checklist}

This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textbf{YES}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results: \textbf{YES}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textbf{YES}
\end{itemize}

Does this paper make theoretical contributions? \textbf{NO}

% If yes, please complete the list below.
% \begin{itemize}
%     \item All assumptions and restrictions are stated clearly and formally. YES
%     \item All novel claims are stated formally (e.g., in theorem statements). YES
%     \item Proofs of all novel claims are included. YES
%     \item Proof sketches or intuitions are given for complex and/or novel results. YES
%     \item Appropriate citations to theoretical tools used are given. YES
%     \item All theoretical claims are demonstrated empirically to hold. YES
%     \item All experimental code used to eliminate or disprove claims is included. YES
% \end{itemize}

Does this paper rely on one or more datasets? \textbf{YES}

If yes, please complete the list below.
\begin{itemize}
    \item  A motivation is given for why the experiments are conducted on the selected datasets. \textbf{YES}
    \item All novel datasets introduced in this paper are included in a data appendix. \textbf{NA}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{NA}
    \item  All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \textbf{YES}
    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \textbf{YES}
    \item  All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \textbf{NA}
\end{itemize}


Does this paper include computational experiments? \textbf{YES}

If yes, please complete the list below.
\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. \textbf{YES}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. \textbf{YES}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \textbf{YES}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \textbf{YES}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \textbf{YES}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \textbf{YES}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \textbf{YES}
    \item This paper states the number of algorithm runs used to compute each reported result. \textbf{YES}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \textbf{YES}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \textbf{NO}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \textbf{NO}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \textbf{YES}
\end{itemize}


% This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/\textbf{no}/NA)

% Answer: The final hyperparameters are included in the supplemental materials.
